S$^{2}$-PINN: Stochastic Separable Physics-Informed Neural Networks

Uncertainty quantification (UQ) for random partial differential equations (PDEs) is ubiquitous in computational science and engineering. However, classical spectral solvers for this class of problems face the curse of dimensionality, and existing neural solvers often ignore the stochastic structure that makes moments and calibration tractable. We introduce a stochastic separable physics-informed neural network, dubbed S$^{2}$-PINN, that represents the solution $u(t,\mathbf{x},\mathbf{Z})$ of a random PDE with a learnable Gaussian spatial dictionary, Fourier temporal features, and a generalized polynomial chaos (gPC) stochastic basis, coupled by a low-rank Canonical Polyadic (CP) tensor decomposition core. The method is trained with a hybrid strong-form and gPC-projected residual loss. Our theoretical analysis establishes that the separable class is dense in $L^2$ under mild conditions, and the projected residual corresponds exactly to a stochastic Galerkin constraint. Furthermore, we show that mini-batch projection coefficients are logarithmically dependent on the number of gPC modes, and that the orthogonality penalty controls the conditioning of the learned spatial dictionary. Using four manufactured random PDE benchmarks, we show that S$^{2}$-PINN outperforms nine baselines in terms of mean and variance accuracy, as well as calibration, while using significantly fewer parameters. Further evaluations on non-manufactured Poisson and Darcy problems, a stochastic Navier--Stokes problem, a diffusion scaling study of higher random dimensions, and two stochastic inverse problems reveal the generalization capabilities of the proposed structure. Together, these results support stochastic separability as an effective design principle for physics-informed neural UQ. The code for the experiments can be found in https://github.com/DMax1314/s2pinn

==> spinn_fig/ablation_tables.tex <==
% Ablation Study Tables
% Auto-generated from results_summary.csv
% DO NOT EDIT MANUALLY - regenerate with generate_ablation_tables.py

% Baseline Architecture Ablation (hidden size × layers)
\begin{table}[t]
\centering
\caption{Baseline Architecture Ablation (hidden size × layers)}
\label{tab:ablation_baseline_arch}
\begin{tabular}{lccc}
\toprule
Configuration & $\mathcal{E}_{\bar{u}}$ & $\mathcal{E}_{u_1}$ & $\mathcal{E}_{u_2}$ \\
\midrule
\textit{default (baseline)} & $(4.23 \pm 1.03) \times 10^{-3}$ & $(3.97 \pm 1.39) \times 10^{-3}$ & $(4.25 \pm 1.07) \times 10^{-3}$ \\
h=128, L=4 & $(4.41 \pm 0.63) \times 10^{-2}$ & $(4.10 \pm 0.34) \times 10^{-2}$ & $(3.86 \pm 0.64) \times 10^{-2}$ \\
h=128, L=6 & \textbf{$(2.33 \pm 0.44) \times 10^{-2}$} & \textbf{$(2.12 \pm 0.44) \times 10^{-2}$} & \textbf{$(2.26 \pm 0.38) \times 10^{-2}$} \\
h=256, L=4 & $(3.26 \pm 1.39) \times 10^{-2}$ & $(3.09 \pm 1.09) \times 10^{-2}$ & $(3.04 \pm 1.01) \times 10^{-2}$ \\
h=256, L=6 & $(6.10 \pm 2.69) \times 10^{-2}$ & $(5.81 \pm 2.56) \times 10^{-2}$ & $(5.68 \pm 2.58) \times 10^{-2}$ \\
\bottomrule
\end{tabular}
\end{table}

% Spatial Atoms (M) Ablation
\begin{table}[t]
\centering
\caption{Spatial Atoms (M) Ablation}
\label{tab:ablation_spatial_atoms}
\begin{tabular}{lccc}
\toprule
Configuration & $\mathcal{E}_{\bar{u}}$ & $\mathcal{E}_{u_1}$ & $\mathcal{E}_{u_2}$ \\
\midrule
\textit{default (baseline)} & $(4.23 \pm 1.03) \times 10^{-3}$ & $(3.97 \pm 1.39) \times 10^{-3}$ & $(4.25 \pm 1.07) \times 10^{-3}$ \\
M=64 & $(9.79 \pm 1.95) \times 10^{-3}$ & $(9.82 \pm 1.89) \times 10^{-3}$ & $(9.77 \pm 1.90) \times 10^{-3}$ \\
M=128 & $(6.11 \pm 1.37) \times 10^{-3}$ & $(6.16 \pm 1.30) \times 10^{-3}$ & $(6.07 \pm 1.30) \times 10^{-3}$ \\
M=512 & \textbf{$(1.91 \pm 0.49) \times 10^{-3}$} & \textbf{$(1.89 \pm 0.39) \times 10^{-3}$} & \textbf{$(1.93 \pm 0.62) \times 10^{-3}$} \\
\bottomrule
\end{tabular}
\end{table}

% Regularization Component Ablation
\begin{table}[t]
\centering
\caption{Regularization Component Ablation}
\label{tab:ablation_regularization}
\begin{tabular}{lccc}
\toprule
Configuration & $\mathcal{E}_{\bar{u}}$ & $\mathcal{E}_{u_1}$ & $\mathcal{E}_{u_2}$ \\
\midrule
\textit{default (baseline)} & $(4.23 \pm 1.03) \times 10^{-3}$ & $(3.97 \pm 1.39) \times 10^{-3}$ & $(4.25 \pm 1.07) \times 10^{-3}$ \\
w/o fac orth & $(3.56 \pm 1.48) \times 10^{-3}$ & $(3.62 \pm 1.28) \times 10^{-3}$ & $(3.62 \pm 1.46) \times 10^{-3}$ \\
w/o gram & $(3.71 \pm 0.34) \times 10^{-3}$ & $(3.44 \pm 0.49) \times 10^{-3}$ & $(3.74 \pm 0.35) \times 10^{-3}$ \\
w/o proj & $(3.17 \pm 0.96) \times 10^{-3}$ & $(3.12 \pm 0.99) \times 10^{-3}$ & \textbf{$(3.15 \pm 0.98) \times 10^{-3}$} \\
w/o reg & \textbf{$(3.15 \pm 0.70) \times 10^{-3}$} & \textbf{$(2.89 \pm 0.76) \times 10^{-3}$} & $(3.29 \pm 0.72) \times 10^{-3}$ \\
\bottomrule
\end{tabular}
\end{table}

% gPC Order (p) Ablation
\begin{table}[t]
\centering
\caption{gPC Order (p) Ablation}
\label{tab:ablation_gpc_order}
\begin{tabular}{lccc}
\toprule
Configuration & $\mathcal{E}_{\bar{u}}$ & $\mathcal{E}_{u_1}$ & $\mathcal{E}_{u_2}$ \\
\midrule
\textit{default (baseline)} & $(4.23 \pm 1.03) \times 10^{-3}$ & $(3.97 \pm 1.39) \times 10^{-3}$ & $(4.25 \pm 1.07) \times 10^{-3}$ \\
p=1 & $(3.85 \pm 1.75) \times 10^{-3}$ & $(4.30 \pm 1.91) \times 10^{-3}$ & $(4.44 \pm 1.68) \times 10^{-3}$ \\
p=2 & \textbf{$(3.50 \pm 1.06) \times 10^{-3}$} & \textbf{$(3.54 \pm 1.03) \times 10^{-3}$} & \textbf{$(3.51 \pm 1.12) \times 10^{-3}$} \\
p=4 & $(2.56 \pm 3.43) \times 10^{-2}$ & $(2.35 \pm 3.08) \times 10^{-2}$ & $(2.55 \pm 3.41) \times 10^{-2}$ \\
\bottomrule
\end{tabular}
\end{table}

% CP Rank (q) Ablation
\begin{table}[t]
\centering
\caption{CP Rank (q) Ablation}
\label{tab:ablation_cp_rank}
\begin{tabular}{lccc}
\toprule
Configuration & $\mathcal{E}_{\bar{u}}$ & $\mathcal{E}_{u_1}$ & $\mathcal{E}_{u_2}$ \\
\midrule
\textit{default (baseline)} & $(4.23 \pm 1.03) \times 10^{-3}$ & $(3.97 \pm 1.39) \times 10^{-3}$ & $(4.25 \pm 1.07) \times 10^{-3}$ \\
q=4 & $(4.74 \pm 1.84) \times 10^{-3}$ & $(4.66 \pm 1.79) \times 10^{-3}$ & $(4.79 \pm 1.89) \times 10^{-3}$ \\
q=8 & \textbf{$(2.80 \pm 1.04) \times 10^{-3}$} & \textbf{$(2.73 \pm 1.09) \times 10^{-3}$} & \textbf{$(2.85 \pm 0.93) \times 10^{-3}$} \\
q=32 & $(3.24 \pm 0.91) \times 10^{-3}$ & $(3.43 \pm 0.42) \times 10^{-3}$ & $(3.15 \pm 0.83) \times 10^{-3}$ \\
\bottomrule
\end{tabular}
\end{table}

